A Comparative Study of Full Apps and Lite Apps for Android

App developers aim to create apps that cater to the needs of different types of users. This development approach, also known as the "one-size-fits-all" strategy, involves combining various functionalities into one app. However, this approach has drawbacks, such as lower conversion rates, slower download speed, larger attack surfaces, and lower update rates. To address these issues, developers have created "lite" versions to attract new users and enhance the user experience. Despite this, there has been no study conducted to examine the relationship between lite and full apps. To address this gap, we present a comparative study of lite apps, exploring the similarities and differences between lite and full apps from various perspectives. Our findings indicate that most existing lite apps fail to fulfill their intended goals (e.g., smaller in size, faster to download, and using less data). Our study also reveals the potential security risks associated with lite apps.

==> discussion.tex <==
\section{Discussion and Insights}
%This section discusses implication from this study. We also list some potential threats to validity in our study.

\subsection{Implication and Research Directions}
The findings and conclusions drawn in this study lead to several potential insights and opportunities for researchers to work on.


%\noindent\textbf{Implication 2: More than a ``lightweight'' version.} Intuitively, lite apps are considered as lightweight versions of full apps. However, our study reveals that sometimes lite apps requires additional permissions, have unique components, specified methods compared to their corresponding full apps. Such results suggest that characteristics and usage scenarios of apps and companion lite apps can also be different. The designs of lite apps can be adjusted to be suitable for different usage scenarios and requirements.

\noindent\textbf{Implication 1: Inconsistency and Privacy Issues in Lite Apps.} The driving force behind the development of lite apps is to offer improved user experience on low-end devices with limited resources such as low memory and processing power. The aim of lite apps is to be smaller in size, faster to download, and consume less data compared to traditional native apps. However, our study found that the majority of existing lite apps fall short of their intended goals. For instance, our results indicate that some dangerous permissions not present in full apps can be introduced in lite apps, and some lite apps also violate privacy policy consistency. Only 24.6\% of the lite apps bring performance improvements compared to full apps. These findings suggest that developers must ensure that their lite apps deliver a seamless user experience, are efficient in their resource usage, and perform well on low-end devices.

\noindent\textbf{Implication 2: (Semi-)automatic Migration from Full Apps to Lite Apps.} As presented in our study, we find that approximately 50\% of the non-code resources, approximately 31\% of code in lite apps are directly reused from the full apps. Moreover, the number of lite apps are still limited on app stores. One possible reason is that developers still have to build the lite apps from scratch. It can be promising to build lite versions of apps by migrating legacy apps. Thus, this is a need for building the lite versions of apps by automatic or semi-automatic migrating existing legacy apps. This also benefits the development of lite apps and boost the lite app ecosystem. Our study shed the light on building such a (semi-)automatic tool.

Our study also suggests several potential research directions for lite apps that could deepen our understanding of this technology and its potential impact:

\noindent\textbf{Research Directions 1: Predicting Lite App Features.} Research should be conducted to predict which functionalities are most critical for lite apps and tailored users with deep learning techniques.

\noindent\textbf{Research Directions 2: Integration with Full App.} Research should be conducted to offer the option to upgrade to the full app for users who need more functionality. 

\noindent\textbf{Research Directions 3: Improving the Data Collection Practices in Lite Apps.} Research should be conducted on exploring alternative monetization models for lite apps that do not rely on data collection, such as subscriptions or in-app purchases.

\subsection{Threats to Validity}
The validity of the results may be impacted by the limited number of app pairs studied. The findings of this study should not be generalized to the entire app ecosystem. The method used, static analysis, may have limitations in accurately analyzing complex language features such as reflection and dynamic loading. However, these language features are not the focus of the similarity comparison, so their impact on the results is minimal. Other factors such as device and network conditions that may affect the results were not controlled for or taken into account in this study.

